Large-scale analysis of user exposure to online advertising in Facebook

Online advertising is the major source of income for a large portion of Internet Services. There exists a body of literature aiming at optimizing ads engagement, understanding the privacy and ethical implications of online advertising, etc. However, to the best of our knowledge, no previous work analyses at large scale the exposure of real users to online advertising. This paper performs a comprehensive analysis of the exposure of users to ads and advertisers using a dataset including more than 7M ads from 140K unique advertisers delivered to more than 5K users that was collected between October 2016 and May 2018. The study focuses on Facebook, which is the second largest advertising platform only to Google in terms of revenue, and accounts for more than 2.2B monthly active users. Our analysis reveals that Facebook users are exposed (in median) to 70 ads per week, which come from 12 advertisers. Ads represent between 10% and 15% of all the information received in users' newsfeed. A small increment of 1% in the portion of ads in the newsfeed could roughly represent a revenue increase of 8.17M USD per week for Facebook. Finally, we also reveal that Facebook users are overprofiled since in the best case only 22.76% of the interests Facebook assigns to users for advertising purpose are actually related to the ads those users receive.

==> limitations.tex <==
\section{Limitations}

To answer the research questions addressed in the paper we have applied a complex methodology that required to implement multiple steps . First, we have implemented a tool, the FDVT, that collects data from FB users who have installed it. Second, we have identified the landing page associated to ads that were delivered in many cases months or even a year before the time we ran the identification process. Third, given the huge volume of data we are analyzing, i.e., more than 7M ads corresponding to more than 140K unique advertisers, we apply a heuristic that links the advertiser to the domain of the landing page (e.g., if the landing page is www.nike.com, we consider the advertiser is Nike). Following, we list the main limitations of the applied methodology and discuss what are their implication in the obtained results. 


(i) In Section \ref{sec:dataset} we reported that we are able to find the advertiser (i.e., retrieve the landing page) for 3/4 of the ads. The two main reasons for not accessing the remaining advertisers is either because the landing page does not exist anymore or the chain of redirections is broken and our crawler get stuck in an intermediate point before reaching the final landing page. Both limitations are mainly due to the fact that we are trying to retrieve the landing page of FDVT ads months or even one year after they were delivered. This limitation mainly affects the results obtained in Section\ref{sec:advertisers}: (i) the number of advertisers that reach users reported in Table \ref{table:2_numberadvertisers} may be actually higher, and (ii) the share of ads coming from the N predominant advertisers may be actually higher than the one shown in Figure \ref{fig:AdverstiserCDF}. Therefore, the results obtained across the section can be considered as a lower bound.   

(ii) Advertisers are identified using the landing page domain. However, in some cases an advertiser may own two or more different domains ('adidas.com', 'adidasbasketball.com', 'adidasrunners.de', 'adidaswatches.com'). In those cases we will consider one advertiser per domain in our analysis rather than a single advertiser. This heuristic affects the same results of Section \ref{sec:advertisers} described before. Hence, this reinforces the message that the results depicted in Table \ref{table:2_numberadvertisers}  and Figure \ref{fig:AdverstiserCDF} are very likely a lower bound.

(iii) The FDVT only works in desktops/laptops. Therefore, it collects all the ads users receive when they connect to Facebook using the desktop/laptop where they have installed the FDVT. However, if users also connect to Facebook using other devices (e.g., mobile phone) we miss all the ads received during that time. So basically for some users (unfortunately we cannot measure which ones) we have a subset of all the ads they have received. This again implies the same concept of lower bound in the same results impacted by the two previous limitations. In addition, Section \ref{sec:engagement} analyzes the engagement of users, i.e., the probability the click in ads of a particular advertiser according the number of ads impressions the user receives from that advertiser. Hence, in this paper we are measuring the engagement probability of FB advertisers in desktops/laptops. We need to be rigorous and we cannot extrapolate the obtained results to mobile devices. However, in case of being able to access a dataset from mobile devices as the one generated from the data collected using the FDVT we could apply the same methodology used in this paper to analyze the mobile environment.







